Negative Control Falsification Tests for Instrumental Variable Designs

The validity of instrumental variable (IV) designs is typically tested using two types of falsification tests. We characterize these tests as conditional independence tests between negative control variables -- proxies for unobserved variables posing a threat to the identification -- and the IV or the outcome. We describe the conditions that variables must satisfy in order to serve as negative controls. We show that these falsification tests examine not only independence and the exclusion restriction, but also functional form assumptions. Our analysis reveals that conventional applications of these tests may flag problems even in valid IV designs. We offer implementation guidance to address these issues.

==> tab_applications_intro.tex <==
\begin{table}[]
    \centering
    %\small    
    \renewcommand{\tabspace}{\\[-1ex]}
    \newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
 \begin{tabular}{@{\extracolsep{3pt}}*5{L{1.6in}}rr}
     \toprule
     &\multicolumn{4}{c}{Original Variable Description} & \multicolumn{2}{c}{\# of Negative Controls}\\
     \cline{2-5} \cline{6-7}
     \tabspace
       & Outcome & Treatment & IV & Negative Controls & \makecell{Original\\Paper} & \makecell{Our\\Analyses} \\
     \midrule
& (1) & (2) & (3) & (4) & (5) & (6)\\ 
\midrule
     \\
     \multicolumn{6}{l}{\textbf{A. Negative Control Outcome Tests}}\\
     \\
     \cite{autor2013china} & Local labor market outcomes &Import competition from China  & Other countries' import competition from China & Lagged local labor market manufacturing employment &3 & 52\\
     \tabspace
     \cite{deming2014using} & Student test scores & Value added of the school  & School assignment lottery, interacted with school VA & No negative control analysis in the original paper & $-$& 37 \\
     \\
     \multicolumn{6}{l}{\textbf{B. Negative Control Instrument Tests}}\\
     \\
     \cite{ashraf2013out} & Level of economic development & Population genetic diversity  & Migratory distance from East Africa & Migratory distance from alternative locations not associated with genetic diversity (e.g., London) & 3 &3\\
     \tabspace
     \cite{nunn2014us} & Level of civil conflict  & Receipt of U.S. food aid & Variation in U.S. wheat production & Variation in U.S. production of crops not associated with aid (e.g., oranges) & 10 & 10\\
     \bottomrule
\end{tabular}

\end{table}


==> tab_applications_nci.tex <==
\begin{table}[]
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{1}{c}{\makecell{\bf Without Conditioning\\\bf on the IV}}& \multicolumn{3}{c}{\makecell{\bf With Conditioning\\\bf on the IV}} & \\
\cline{2-2} \cline{3-5}
\tabspace
& \makecell{Single\\linear model} & \makecell{Single \\linear model} & \makecell{Multiple\\linear models} & \makecell{\\F-Test} & \multicolumn{1}{c}{\makecell{Number of\\Observations}} \\
\midrule
& (1) & (2) & (3) & (4) & (5)\\ 
\midrule
\cite{nunn2014us} & 0.007 & 0.123 & 0.636 & 0.138 & 4572 \\
\cite{ashraf2013out} & 0.234 & 0.778 & 1.000 & 0.994 & 145 \\
\bottomrule
\end{tabular}
\label{tab:your_table_label}
\end{table}

==> tab_applications_nco.tex <==
\begin{table}[]
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{\extracolsep{3pt}}l*{7}{c}}
\toprule
 & \makecell{\bf Original\\\bf Analysis}  & \multicolumn{5}{c}{\bf Alternative Analyses}  \\ 
\cline{2-2} \cline{3-7}
 \tabspace
\textit{Type of Test:}& \makecell[b]{Single\\linear model\\without controls} &   \makecell[b]{Single\\linear model\\} & \makecell[b]{Multiple\\linear models\\} & \makecell[b]{F-Test\\} & \makecell[b]{GAM, \\Linear\\Controls} & \makecell[b]{GAM,\\Nonlinear\\Controls} &  \makecell[b]{Number of\\Observations} \\

 \midrule
  & (1) & (2) & (3) & (4) & (5) & (6) & (7)  \\
 \midrule
  \cite{autor2013china} & 0.004 &   0.593 & $<$0.001 & $<$0.001 & 1.000 & 1.000 & 722 \\
\cite{deming2014using}  & - &   0.686 & $<$0.001 & $<$0.001 & $<$0.001 & $<$0.001 & 2343 \\
%\citeauthor{deming2014using} (Alternative IV) & -  & 0.452 & 0.101 & 0.648 & 1.000 & 1.000 & 2343 \\ 
\bottomrule
\end{tabular}
\end{table}


==> tab_ashraf_galor.tex <==


\renewcommand{\arraystretch}{1.5}

\begin{table}[H]
    \centering
    \caption{Ashraf \& Galor analysis. The reported results are p-values. In the `separate` column, the NCIV was included linearly and quadratically (as in the original analysis). In the `Wald` column we performed the Wald test with robust s.e. for both linear and quadratic terms. In the `GAM` column, we fitted a GAM with a smooth NCIV term and tested with Wald posthoc test with robust s.e..}
    \begin{tabular}{lllllll}
    \toprule
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{Seperate (lin, quad)} & \multicolumn{2}{c}{Wald} & \multicolumn{2}{c}{GAM} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{IV Adj.} & \multicolumn{2}{c}{IV Adj.} & \multicolumn{2}{c}{IV Adj.} \\
    \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
     & FALSE & TRUE & FALSE & TRUE & FALSE & TRUE\\
    \midrule
    Addis Ababa & 0.034, <0.01 & 0.284, 0.104 & <0.01 & 0.017 & <0.01 & 1\\
    London & 0.544, 0.441 & 0.268, 0.226 & <0.01 & 0.411 & <0.01 & 1\\
    Mexico & 0.542, 0.234 & 0.974, 0.778 & <0.01 & 0.745 & <0.01 & 0.994\\
    Tokyo & 0.762, 0.47 & 0.889, 0.827 & 0.215 & 0.786 & <0.01 & 0.994\\
    \bottomrule
    \end{tabular}
\end{table}



==> tab_autor_nc_diagnostics.tex <==
Population count & 0.093 & 0.028\\
Size of 1990 workforce & 0.085 & 0.031\\
Share of employment & 0.094 & 0.006\\
Share of employment in manufacturing & 0.424 & 0.146\\
Share of employment in manufacturing of males & 0.324 & 0.098\\
Share of employment in manufacturing of females & 0.454 & 0.174\\
Share of employment in manufacturing no college education & 0.442 & 0.100\\
Share of employment in manufacturing with college education & 0.263 & 0.159\\
Share of employment in manufacturing ages 16-34 & 0.371 & 0.101\\
Share of employment in manufacturing ages 35-49 & 0.404 & 0.183\\
Share of employment in manufacturing ages 50-64 & 0.421 & 0.126\\
Share of employment in non-manufacturing & 0.289 & 0.134\\
Share of employment in non-manufacturing of males & 0.241 & 0.099\\
Share of employment in non-manufacturing of females & 0.285 & 0.150\\
Share of employment in non-manufacturing no college education & 0.304 & 0.096\\
Share of employment in non-manufacturing with college education & 0.178 & 0.137\\
Share of employment in non-manufacturing ages 16-34 & 0.214 & 0.081\\
Share of employment in non-manufacturing ages 35-49 & 0.304 & 0.181\\
Share of employment in non-manufacturing ages 50-64 & 0.242 & 0.087\\
Share of unemployment & 0.010 & 0.026\\
Share of unemployment of males & 0.003 & 0.017\\
Share of unemployment of females & 0.031 & 0.033\\
Share of unemployment no college education & 0.005 & 0.024\\
Share of unemployment with college education & 0.015 & 0.034\\
Share of unemployment ages 16-34 & 0.023 & 0.017\\
Share of unemployment ages 35-49 & 0.021 & 0.047\\
Share of unemployment ages 50-64 & 0.034 & 0.017\\
Share of NILF & 0.112 & 0.002\\
Share of NILF of males & 0.045 & 0.009\\
Share of NILF of females & 0.168 & 0.023\\
Share of NILF no college education & 0.171 & 0.014\\
Share of NILF with college education & 0.022 & 0.013\\
Share of NILF ages 16-34 & 0.081 & 0.002\\
Share of NILF ages 35-49 & 0.147 & 0.017\\
Share of NILF ages 50-64 & 0.050 & 0.000\\
Share of SSDI recipt in 1990 & 0.028 & 0.005\\
Average log weekly wage in manufacturing & 0.109 & 0.012\\
Average log weekly wage in non-manufacturing & 0.023 & 0.021\\
Total individual transfers & 0.155 & 0.031\\
Medical benefits & 0.160 & 0.011\\
Federal income assist & 0.048 & 0.040\\
Other assist & 0.055 & 0.017\\
Unemployment benefits & 0.094 & 0.014\\
Trade Adjustment Assistance benefits & 0.037 & 0.029\\
Education or training assistance & 0.061 & 0.068\\
Social security retirement benefits & 0.083 & 0.031\\
Social security disability benefits & 0.015 & 0.017\\
Average Total income & 0.018 & 0.001\\
Average wage-salary & 0.038 & 0.042\\
Year 1990 outcome & 0.175 & 0.097\\
Year 1980 outcome & 0.018 & 0.018\\
Year 1970 outcome & 0.031 & 0.014\\

==> tab_autor_results.tex <==

\renewcommand{\arraystretch}{1.5}
\begin{table}[H]
	\centering
	\captionsetup{width=.8\linewidth}
	\begin{tabular}{p{3in}*{5}{p{.8in}}}
		\toprule
		&\multicolumn{5}{c}{Instrument: ($\Delta$ imports from China to other countries)$/$worker}\\
		p-values &\multicolumn{5}{c}{\textit{Specification}}\\
		\cline{2-6}
		 & (1) & (2) & (3) & (4) & (5) \\
		\midrule
		\textbf{Method:}\\
		~~~F-test & 0.046 & 0.027 & 0.01 & <0.01 & <0.01\\
		~~~Bonferroni & <0.01 & <0.01 & <0.01 & <0.01 & <0.01\\
  		~~~GAM & <0.01 & <0.01 & <0.01 & <0.01 & <0.01\\
        ~~~Linear -- Single Negative Control (1970 Outcome)& 0.246 & 0.857 & 0.47 & 0.864 & 0.574\\
        ~~~GAM -- Single NC (1970 Outcome) & <0.01 & 0.028 & 0.017 &<0.01 & 0.011\\ 
%		~~~Random Forests & <0.01 & 0.43 & 0.54 & 0.76 & 0.89\\
		\midrule
		\textbf{Negative Control Variables:}\\
		&\multicolumn{5}{c}{pre-1990 variables}\\
		\textbf{Control Variables:}\\
		\% of Employment in Manufacturing & Yes & Yes & Yes & Yes & Yes\\
		\% College Educated &  &  & Yes &  & Yes\\
		\% Foreign Born &  &  & Yes &  & Yes\\
		\% Female Employment &  &  & Yes &  & Yes\\
		\% Employment in Routine Occupations &  &  &  & Yes & Yes\\
		Average offshorability index of occupations &  &  &  & Yes & Yes\\
		Census Division Dummies &  & Yes & Yes & Yes & Yes\\
		\bottomrule

	\end{tabular}
\end{table}

%
%\begin{table}
%    \centering
%    \begin{tabular}{llllll}
%\toprule
%Method (Bonf $\equiv$ F-test) & Control2 & Control3 & Control4 & Control5 & Control6\\
%\midrule
%NC=outcome1970 & 0.246 & 0.828 & 0.683 & 0.747 & 0.709\\
%\bottomrule
%\end{tabular}
%\end{table}

==> tab_intro_examples.tex <==
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{*3{>{\raggedright\arraybackslash}p{.15\textwidth}}*3{>{\raggedright\arraybackslash}p{.30\textwidth}}}
\multicolumn{5}{l}{\textbf{A. Negative Control Outcome Tests}} \\
\midrule
\textbf{Paper} & \textbf{Treatment} & \textbf{Outcome} & \textbf{IV} & \textbf{Threat} & \textbf{NCO (IV should not be correlated with it)} \\
\midrule
\citet{martin2017bias} & Fox News viewership & Republican vote share in 2008 & Channel position: Lower channel numbers induce larger viewership & Cable companies might place Fox News in lower channels in more conservative locations  & Republican vote share in 1996\\
%\citet{fredriksson2013long} & Class size & Log wages & Expected class size based on cohort size and maximum class size: Maximum class rule triggers the opening of an additional class when cohort size exceeds a threshold & High ability/SES families might be able to manipulate cohort size & Verify that expected class size is uncorrelated with parental income \\
\citet{angrist1996children} & Number of children & Female labor supply & Same-sex sibship: Families with same-sex sibship for the first two children are more likely to have more children & Same-sex sibship may increase hand-me-downs, reducing expenditures and potentially labor supply & Clothing expenditure   \citep{rosenzweig2000natural} \\
\citet{autor2013china} & Shift-share based on import penetration in US & Manufacturing employment & Shift-share based on import penetration in non-US developed countries%: Import in non-US countries will be correlated with supply factors from China and not demand factors from US
& Commuting zones with importing industries  might be declining for other reasons & Manufacturing employment trends before large Chinese import competition\\
\citet{doyle2015measuring,chan2023there} & Hospital assignment & Health outcomes & Ambulance company assignment, which strongly predicts  hospital assignment & Patient ambulance assignment may depend on their health & Patient demographics \\
\citet{jager2022substitutable} & Worker exits & Incumbent workers' wages & Unexpected worker deaths in small firms & Worker death could be correlated with firm-specific risks, which affect wages & Worker unexpected deaths in same firms in other years \\

\tabspace
\multicolumn{5}{l}{\textbf{B. Negative Control Instrument Tests}}\\
\midrule
\textbf{Paper} & \textbf{Treatment} & \textbf{Outcome} & \textbf{IV} & \textbf{Threat} &\textbf{NCI (conditional on IV, outcome should not be correlated with it)}\\
\midrule
\citet{nunn2014us} & US food aid & Conflict in recipient countries & Wheat production: US food aid increases when it booms & Wheat production is affected by weather conditions, which could also have other impacts on conflicts & Production of crops not used for aid (e.g., oranges) \\
%\citet{acemoglu2020weak} & Socialist organization (Peasant Fasci) & Sicilian Mafia presence & The 1893 drought: Led to increase in support for socialist organizations & Weather conditions might generate convenient economic conditions for Mafia emergence & Rainfall in previous years \\
\citet{ashraf2013out} & Genetic diversity & Economic development & Distance from Addis Ababa, which predicts genetic diversity due to the human origin hypothesis & Other economic factors have geographical dispersion & Distance from other cities (e.g., London, Mexico City) \\

\citet{de2020consumption} & Peer consumption & Own consumption & Shocks in firms of distant peers: Negative shocks in firms of distant peers are less likely to be correlated with self economic shocks & Shocks to larger firms are statistically more likely to affect distant peers, and might also affect consumption in other ways & Placebo shocks: Calculate same IV based on permutated employer-employee relationship (keeping employer size unchanged) \\
\citet{madestam2013political} & Tea Party protest participation & Republican vote & Rain on April 15, 2009, which affected local participation in one of the first large Tea Party protests & Probability of rain is driven by local climate conditions, which could relate to voting in various ways & Rain on other dates \\
\bottomrule
\end{tabular}


==> tab_survey.tex <==
\begin{table}[]
\begin{tabular}{@{\extracolsep{3pt}}l*{9}{ >{\centering\arraybackslash}p{.87in}}}
\toprule
&&& \multicolumn{6}{c}{\makecell{Falsification Test Characteristics\\(Share of Papers that Included Falsification Tests)}}\\
\cline{4-9}
\tabspace
&&& \multicolumn{3}{c}{Type of Test} & \multicolumn{3}{c}{Test Specification} &    \\                 
\cline{4-6} \cline{7-9}  
\tabspace
      & \makecell[b]{Papers\\Reviewed} 
      & \makecell[b]{Share with\\Falsification\\Tests} 
      & \makecell[b]{Negative\\Control\\Outcome}  
      & \makecell[b]{Negative\\Control\\Instrument}  
      & \makecell[b]{Other} 
      & \makecell[b]{Replace\\Outcome\\with\\NCO} 
      & \makecell[b]{Replace\\IV\\with\\NCI} 
      & \makecell[b]{Add NCI to\\reduced-\\form} 
      & \makecell[b]{\# Negative\\Controls\\Used\\(median)} \\ 
\midrule
& (1)  & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\
\midrule

All & 140 & 0.51 & 0.75 & 0.24 & 0.21 & 0.43 & 0.18 & 0.06 & 3.50 \\ 
   \textit{by Journal:}\\REStud &  48 & 0.42 & 0.75 & 0.40 & 0.10 & 0.65 & 0.35 & 0.05 & 4.00 \\ 
  AER &  42 & 0.50 & 0.86 & 0.24 & 0.05 & 0.57 & 0.24 & 0.00 & 4.00 \\ 
  JPE &  21 & 0.62 & 0.62 & 0.15 & 0.31 & 0.23 & 0.00 & 0.15 & 3.50 \\ 
  QJE &  19 & 0.68 & 0.77 & 0.15 & 0.46 & 0.15 & 0.08 & 0.08 & 2.00 \\ 
  ECMA &  10 & 0.50 & 0.60 & 0.00 & 0.40 & 0.20 & 0.00 & 0.00 & 4.50 \\ 

\bottomrule
\end{tabular}
\end{table}

